Cohomology fractals, Cannon-Thurston maps, and the geodesic flow

Cohomology fractals are images naturally associated to cohomology classes in hyperbolic three-manifolds. We generate these images for cusped, incomplete, and closed hyperbolic three-manifolds in real-time by ray-tracing to a fixed visual radius. We discovered cohomology fractals while attempting to illustrate Cannon-Thurston maps without using vector graphics; we prove a correspondence between these two, when the cohomology class is dual to a fibration. This allows us to verify our implementations by comparing our images of cohomology fractals to existing pictures of Cannon-Thurston maps. In a sequence of experiments, we explore the limiting behaviour of cohomology fractals as the visual radius increases. Motivated by these experiments, we prove that the values of the cohomology fractals are normally distributed, but with diverging standard deviations. In fact, the cohomology fractals do not converge to a function in the limit. Instead, we show that the limit is a distribution on the sphere at infinity, only depending on the manifold and cohomology class.

==> header_article.tex <==
%%% Environments %%%

% Numbering
% see http://tex.stackexchange.com/questions/41299/how-to-identify-the-counter-of-equation-theorem-and-section

\makeatletter
\let\c@equation\c@subsection
\makeatother
\numberwithin{equation}{section} 

\makeatletter
\let\c@figure\c@equation
\makeatother
\numberwithin{figure}{section} 

% Formatting 
% see amsthdoc.pdf for general discussion. 

% \swapnumbers 

% It is Bourbaki style to put labels (numbering) before the <type>.
% This is used in various places - eg Dunfield recently, Bridson and
% Haefliger.  Suggested, but not used, by Bernstein
% (http://cr.yp.to/writing.html).  If you fix the non-bold/bold/italic
% problem (three typefaces in three words arrgh!) then it looks
% better.  But it doesn't match usage in the text, and I think that
% controls...  Perhaps if the numbers could be placed in the margin in
% a nice way?  But then there would be a ragged left.

\theoremstyle{plain}
\newtheorem{theorem}[equation]{Theorem}
\newtheorem{corollary}[equation]{Corollary}
\newtheorem{lemma}[equation]{Lemma}
\newtheorem{conjecture}[equation]{Conjecture}
\newtheorem{proposition}[equation]{Proposition}
\newtheorem{principle}[equation]{Principle}
\newtheorem{axiom}[equation]{Axiom}
\newtheorem{ourrule}[equation]{Rule}

\theoremstyle{definition}
\newtheorem{definition/}[equation]{Definition}
\newtheorem{problem}[equation]{Problem}
\newtheorem{solution}[equation]{Solution}
\newtheorem{exercise}[equation]{Exercise}
\newtheorem{example/}[equation]{Example}
\newtheorem{fact}[equation]{Fact}
\newtheorem{question/}[equation]{Question}
\newtheorem{project/}[equation]{Project}
\newtheorem*{question*}{Question}
\newtheorem*{answer*}{Answer}
\newtheorem*{application*}{Application}
\newtheorem{algorithm/}[equation]{Algorithm}
\newtheorem{heuristic/}[equation]{Heuristic}

%%% https://tex.stackexchange.com/questions/291346/marking-the-end-of-a-definition
%%% Using egreg's solution
\newenvironment{definition}
  {\renewcommand{\qedsymbol}{$\Diamond$}%
   \pushQED{\qed}\begin{definition/}}
  {\popQED\end{definition/}}

\newenvironment{example}
  {\renewcommand{\qedsymbol}{$\Diamond$}%
   \pushQED{\qed}\begin{example/}}
  {\popQED\end{example/}}

\newenvironment{question}
  {\renewcommand{\qedsymbol}{$\Diamond$}%
   \pushQED{\qed}\begin{question/}}
  {\popQED\end{question/}}

\newenvironment{project}
  {\renewcommand{\qedsymbol}{$\Diamond$}%
   \pushQED{\qed}\begin{project/}}
  {\popQED\end{project/}}

\newenvironment{algorithm}
  {\renewcommand{\qedsymbol}{$\Diamond$}%
   \pushQED{\qed}\begin{algorithm/}}
  {\popQED\end{algorithm/}}

\newenvironment{heuristic}
  {\renewcommand{\qedsymbol}{$\Diamond$}%
   \pushQED{\qed}\begin{heuristic/}}
  {\popQED\end{heuristic/}}

\theoremstyle{remark}
\newtheorem{remark/}[equation]{Remark}
\newtheorem*{remark*}{Remark}
\newtheorem{remarks}[equation]{Remarks}
\newtheorem{case}{Case}
\newtheorem*{case*}{Case}
\renewcommand{\thecase}{\Roman{case}}
\newtheorem{claim}[equation]{Claim}
\newtheorem*{claim*}{Claim}
\newtheorem*{proofclaim}{Claim}
\newtheorem*{proofsubclaim}{Subclaim}

\newenvironment{remark}
  {\renewcommand{\qedsymbol}{$\Diamond$}%
   \pushQED{\qed}\begin{remark/}}
  {\popQED\end{remark/}}

%%% Refs
\newcommand{\refsec}[1]{Section~\ref{Sec:#1}}
\newcommand{\refapp}[1]{Appendix~\ref{App:#1}}
\newcommand{\refthm}[1]{Theorem~\ref{Thm:#1}}
\newcommand{\refcor}[1]{Corollary~\ref{Cor:#1}}
\newcommand{\reflem}[1]{Lemma~\ref{Lem:#1}}
\newcommand{\refprop}[1]{Proposition~\ref{Prop:#1}}
\newcommand{\refclm}[1]{Claim~\ref{Clm:#1}}
\newcommand{\refrem}[1]{Remark~\ref{Rem:#1}}
\newcommand{\refexa}[1]{Example~\ref{Exa:#1}}
\newcommand{\reffac}[1]{Fact~\ref{Fac:#1}}
\newcommand{\refexe}[1]{Exercise~\ref{Exe:#1}}
\newcommand{\reffig}[1]{Figure~\ref{Fig:#1}}
\newcommand{\reftab}[1]{Table~\ref{Tab:#1}}
\newcommand{\refdef}[1]{Definition~\ref{Def:#1}}
\newcommand{\refprob}[1]{Problem~\ref{Prob:#1}}
\newcommand{\refalg}[1]{Algorithm~\ref{Alg:#1}}
\newcommand{\refax}[1]{Axiom~\ref{Ax:#1}}
\newcommand{\refrul}[1]{Rule~\ref{Rul:#1}}
\newcommand{\refeqn}[1]{Equation~\ref{Eqn:#1}}
\newcommand{\refconj}[1]{Conjecture~\ref{Conj:#1}}
\newcommand{\refobj}[1]{Objective~\ref{Obj:#1}}
\newcommand{\refitm}[1]{(\ref{Itm:#1})}
\newcommand{\refcon}[1]{(\ref{Con:#1})} % conclusion
\newcommand{\refque}[1]{Question~\ref{Que:#1}}

